Schroedinger Operator with Strong Magnetic Field near Boundary

We consider 2-dimensional Schroedinger operator with the non-degenerating magnetic field in the domain with the boundary and under certain non-degeneracy assumptions we derive spectral asymptotics with the remainder estimate better than $O(h^{-1})$, up to $O(\mu^{-1}h^{-1})$ and the principal part $\asymp h^{-2}$ where $h\ll 1$ is Planck constant and $\mu \gg 1$ is the intensity of the magnetic field; $\mu h \le 1$. We also consider generalized Schr\"odinger-Pauli operator in the same framework albeit with $\mu h\ge 1$ and derive spectral asymptotics with the remainder estimate up to O(1) and with the principal part $\asymp \mu h^{-1}$, or, under certain special circumstances with the principal part $\asymp \mu^{1/2} h^{-1/2}$.

==> IRO21/defines_IRO21.tex <==




\hyphenation{%
mic-ro-hy-per-bo-li-ci-ty}  % why doesn't this work?}


\renewcommand{\thefootnote}{{\arabic{footnote})}}
%


%
%%% Theorem-like environments
%
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[chapter]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{condition}[theorem]{Condition}

%

\theoremstyle{definition}


\newtheorem{definition}[theorem]{Definition}
\newtheorem{Problem}[theorem]{Problem}
%
\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}
\newtheorem*{remarknn}{Remark}           % remark with no number
\newtheorem{example}[theorem]{Example}
\newtheorem{problem}[theorem]{Problem}

\numberwithin{equation}{chapter}




\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{it}



\newcommand{\cA}{\mathcal{A}}
 \newcommand{\cB}{\mathcal{B}}
 \newcommand{\cC}{\mathcal{C}}
 \newcommand{\cD}{\mathcal{D}}
 \newcommand{\cE}{\mathcal{E}}
 \newcommand{\cF}{\mathcal{F}}
 \newcommand{\cG}{\mathcal{G}}
 \newcommand{\cH}{\mathcal{H}}
 \newcommand{\cI}{\mathcal{I}}
 \newcommand{\cJ}{\mathcal{J}}
 \newcommand{\cK}{\mathcal{K}}
 \newcommand{\cL}{\mathcal{L}}
 \newcommand{\cM}{\mathcal{M}}
 \newcommand{\cN}{\mathcal{N}}
 \newcommand{\cO}{\mathcal{O}}
 \newcommand{\cP}{\mathcal{P}}
 \newcommand{\cR}{\mathcal{R}}
 \newcommand{\cQ}{\mathcal{Q}}
 \newcommand{\cS}{\mathcal{S}}
 \newcommand{\cT}{\mathcal{T}}
 \newcommand{\cU}{\mathcal{U}}
 \newcommand{\cV}{\mathcal{V}}
 \newcommand{\cW}{\mathcal{W}}
 \newcommand{\cX}{\mathcal{X}}
 \newcommand{\cY}{\mathcal{Y}}
 \newcommand{\cZ}{\mathcal{Z}}

\newcommand{\sA}{\mathscr{A}}
 \newcommand{\sB}{\mathscr{B}}
 \newcommand{\sC}{\mathscr{C}}
 \newcommand{\sD}{\mathscr{D}}
 \newcommand{\sE}{\mathscr{E}}
 \newcommand{\sF}{\mathscr{F}}
 \newcommand{\sG}{\mathscr{G}}
 \newcommand{\sH}{\mathscr{H}}
 \newcommand{\sI}{\mathscr{I}}
 \newcommand{\sJ}{\mathscr{J}}
 \newcommand{\sK}{\mathscr{K}}
 \newcommand{\sL}{\mathscr{L}}
 \newcommand{\sM}{\mathscr{M}}
 \newcommand{\sN}{\mathscr{N}}
 \newcommand{\sO}{\mathscr{O}}
 \newcommand{\sS}{\mathscr{S}}



\newcommand{\an}{{\mathsf{an}}}
\newcommand{\inter}{{\mathsf{int}}}
\newcommand{\inn}{{\mathsf{inn}}}

\newcommand{\bound}{{\mathsf{bound}}}
\newcommand{\even}{{\mathsf{even}}}
\newcommand{\st}{{\mathsf{st}}}

\newcommand{\odd}{{\mathsf{odd}}}
%\newcommand{\even}{{\mathsf{even}}}

\newcommand{\Weyl}{{\mathsf{Weyl}}}


\newcommand{\corr}{{\mathsf{corr}}}
\renewcommand{\d}{{\mathsf{d}}}
\newcommand{\D}{{\mathsf{D}}}
\newcommand{\ext}{{\mathsf{ext}}}
\newcommand{\HS}{{\mathsf{HS}}}
\newcommand{\M}{{\mathsf{M}}}
\newcommand{\m}{{\mathsf{m}}}
\newcommand{\MW}{{\mathsf{MW}}}
\newcommand{\N}{{\mathsf{N}}}
\newcommand{\I}{{\mathsf{I}}}
\newcommand{\J}{{\mathsf{J}}}
\newcommand{\R}{{\mathsf{R}}}
\renewcommand{\S}{{\mathsf{S}}}
\newcommand{\T}{{\mathsf{T}}}
\newcommand{\trans}{{\mathsf{trans}}}
\newcommand{\sU}{{\mathsf{U}}}
\newcommand{\W}{{{\mathsf{W}}}}
\newcommand{\w}{{\mathsf{w}}}
\newcommand{\x}{{\mathsf{x}}}
\newcommand{\cl}{{{\mathsf{cl}}}}
\newcommand{\cone}{{{\mathsf{cone}}}}
\newcommand{\const}{{\mathsf{const}}}
\newcommand{\dist}{{{\mathsf{dist}}}}
\newcommand{\double}{{{\mathsf{double}}}}
\newcommand{\eff}{{{\mathsf{eff}}}}
\newcommand{\elli}{{{\mathsf{ell}}}}
\newcommand{\ess}{{{\mathsf{ess}}}}

\newcommand{\loc}{{{\mathsf{loc}}}}
\newcommand{\new}{{{\mathsf{new}}}}
\newcommand{\old}{{{\mathsf{old}}}}
\newcommand{\reg}{{{\mathsf{reg}}}}
\newcommand{\qreg}{{{\mathsf{qreg}}}}
\newcommand{\cusp}{{{\mathsf{cusp}}}}
\newcommand{\ff}{{{\mathsf{ff}}}}

\newcommand{\per}{{\mathsf{per}}}




\newcommand{\bB}{{\mathbb{B}}}
\newcommand{\bC}{{\mathbb{C}}}
\newcommand{\bH}{{\mathbb{H}}}
\newcommand{\bK}{{\mathbb{K}}}
\newcommand{\bN}{{\mathbb{N}}}
\newcommand{\bQ}{{\mathbb{Q}}}
\newcommand{\bR}{{\mathbb{R}}}
\newcommand{\bS}{{\mathbb{S}}}
\newcommand{\bT}{{\mathbb{T}}}
\newcommand{\bZ}{{\mathbb{Z}}}

\newcommand{\fC}{{\mathfrak{C}}}
\newcommand{\fD}{{\mathfrak{D}}}
\newcommand{\fH}{{\mathfrak{H}}}
\newcommand{\fK}{{\mathfrak{K}}}
\newcommand{\fM}{{\mathfrak{M}}}
\newcommand{\fN}{{\mathfrak{N}}}
\newcommand{\fR}{{\mathfrak{R}}}
\newcommand{\fZ}{{\mathfrak{Z}}}
\newcommand{\fz}{{\mathfrak{z}}}


\def\1{\boldsymbol {|}}
%
%
%%% Bold symbols
%
\newcommand{\boldalpha}{{\boldsymbol{\alpha}}}
\newcommand{\boldbeta}{{\boldsymbol{\beta}}}
\newcommand{\boldgamma}{{\boldsymbol{\gamma}}}
\newcommand{\boldiota}{{\boldsymbol{\iota}}}
\newcommand{\boldlambda}{{\boldsymbol{\lambda}}}
\newcommand{\boldnu}{{\boldsymbol{\nu}}}
\newcommand{\boldpi}{{\boldsymbol{\pi}}}
\newcommand{\boldrho}{{\boldsymbol{\rho}}}

\newcommand{\boldsigma}{{\boldsymbol{\sigma}}}

\newcommand{\boldtau}{{\boldsymbol{\tau}}}


\newcommand{\boldPhi}{{\boldsymbol{\Phi}}}
\newcommand{\boldPsi}{{\boldsymbol{\Psi}}}
%
\newcommand{\blangle}{{\boldsymbol{\langle}}}
\newcommand{\brangle}{{\boldsymbol{\rangle}}}

\newcommand{\bi}{{\bar\imath}}
\newcommand{\bj}{{\bar\jmath}}
\newcommand{\hi}{{\hat\imath}}
\newcommand{\hj}{{\hat\jmath}}
\newcommand{\ti}{{\tilde\imath}}
\newcommand{\tj}{{\tilde\jmath}}
%
%
%%% Compound symbols
%
%
%\newcommand{\2}{{|\!|}}
\newcommand{\3}{{|\!|\!|}}
\newcommand{\Def}{\mathrel{\mathop:}=}
\newcommand{\Fed}{=\mathrel{\mathop:}}


\newcommand{\Ad}{\operatorname{Ad}}
\newcommand{\WF}{\operatorname{WF}}
\newcommand{\Char}{\operatorname{Char}}
\newcommand{\codim}{\operatorname{codim}}
\newcommand{\degen}{{\operatorname{deg}}}     % \deg already defined
\newcommand{\diag}{\operatorname{diag}}
\newcommand{\diam}{\operatorname{diam}}

\newcommand{\graph}{\operatorname{graph}}
\newcommand{\ord}{{{\operatorname  {ord}}}}
\newcommand{\sing}{{{\operatorname  {sing}}}}
%
\newcommand{\Hess}{\operatorname{Hess}}
\renewcommand{\Im}{\operatorname{Im}}       % \Im is already frak I


\newcommand{\Hom}{\operatorname{Hom}}
\newcommand{\indM}{\operatorname{ind_\M}}
\newcommand{\Ker}{\operatorname{Ker}}
\newcommand{\mes}{\operatorname{mes}}
\newcommand{\OO}{\operatorname{O}}
\newcommand{\Op}{\operatorname{Op}}
\newcommand{\osc}{\operatorname{osc}}
\newcommand{\Ran}{\operatorname{Ran}}
\newcommand{\rank}{\operatorname{rank}}
\renewcommand{\Re}{\operatorname{Re}}       % \Re is already frak R
%
\newcommand{\sgn}{\operatorname{sgn}}
\newcommand{\sign}{\operatorname{sign}}
\newcommand{\SO}{\operatorname{SO}}
\newcommand{\Spec}{\operatorname{Spec}}
\newcommand{\Span}{\operatorname{Span}}
%
\newcommand{\Specess}{\operatorname{Spec_\ess}}
\newcommand{\supp}{\operatorname{supp}}
\newcommand{\symb}{\operatorname{symb}}
\newcommand{\tr}{\operatorname{tr}}
\newcommand{\Tr}{\operatorname{Tr}}
\newcommand{\vrai}{\operatorname{vrai}}
%
\newcommand{\Res}{\operatorname{Res}}
\newcommand{\ResR}{\operatorname{Res_\bR}}
\newcommand{\Vol}{\operatorname{vol}}

\newcommand{\trsup}[1]{\operatorname{tr^{#1}}}
%%\def\Hes_#1{\operatorname{Hess_{#1}}}
%\newcommand{\HesSub}[1]{\operatorname{Hess_{#1}}}
%\newcommand{\Hessigma}{\operatorname{Hess^\sigma}}
%
%
%
%
\newenvironment{claim}[1][{\textup{(\theequation)}}]{\refstepcounter{equation}\vglue10pt
\begin{trivlist}
\item[{\hskip\labelsep#1}]}{\vglue10pt\end{trivlist}}


\newenvironment{claim*}[1][{}]{\vglue10pt
\begin{trivlist}
\item[{\hskip\labelsep#1}]}{\vglue10pt\end{trivlist}}

%
%
\newenvironment{phantomequation}[1][]{\refstepcounter{equation}}{}
%
\newcounter{note}

\newenvironment{note}[1]{\refstepcounter{note}{\color{red}$^{\thenote}$}\reversemarginpar
\marginpar{ \hskip-40pt\colorbox{yellow}{\begin{minipage}{70pt} {\color{red}$^{\thenote}$\ #1}\end{minipage}}}}

\newenvironment{Note}[1]{\refstepcounter{note}{$^{\thenote}$}\reversemarginpar
\marginpar{\hskip-40pt\fbox{\begin{minipage}{79pt} {$^{\thenote}$\  #1}\end{minipage}}}}

\DeclareTextCommand{\textinfty}{PU}{\9042\036}



\DeclareTextCommand{\textge}{PU}{\9042\145}
\DeclareTextCommand{\textle}{PU}{\9042\144}
\DeclareTextCommand{\texthat}{PD1}{\136}


%
%\newenvironment{highlight}[1]{\colorbox{yellow}{#1}}
%
%\newenvironment{claim*}[1]{\smallskip
%\begin{trivlist}
%\item[{\hskip\labelsep#1}]}{\smallskip\end{trivlist}}
%
%\newenvironment{pdeq}[1][]{\refstepcounter{equation}}{}
%
%%%% Local Variables:
%%%% mode: latex
%%%% TeX-master: "book"
%%%% End:
%
%

